Mixed Correlator Dispersive CFT Sum Rules

Conformal field theory (CFT) dispersion relations reconstruct correlators in terms of their double discontinuity. When applied to the crossing equation, such dispersive transforms lead to sum rules that suppress the double-twist sector of the spectrum and enjoy positivity properties at large twist. In this paper, we construct dispersive CFT functionals for correlators of unequal scalar operators in position- and Mellin-space. We then evaluate these functionals in the Regge limit to construct mixed correlator holographic CFT functionals which probe scalar particle scattering in Anti-de Sitter spacetime. Finally, we test properties of these dispersive sum rules when applied to the 3D Ising model, and we use truncated sum rules to find approximate solutions to the crossing equation.

==> mixed-correlator-dispersive-sum-rule <==
\contentsline {section}{\numberline {1}Introduction}{2}{section.1}%
\contentsline {section}{\numberline {2}Overview of dispersive CFT sum rules}{3}{section.2}%
\contentsline {section}{\numberline {3}Position-space functionals}{6}{section.3}%
\contentsline {subsection}{\numberline {3.1}Generalities}{6}{subsection.3.1}%
\contentsline {subsection}{\numberline {3.2}Deriving the position-space $\mathfrak {B}_{\mathbf {k}|mn}^{\mathfrak {a},\mathfrak {b}}$ kernel}{8}{subsection.3.2}%
\contentsline {subsection}{\numberline {3.3}Convergence and positivity properties: a plethora of subtraction schemes}{13}{subsection.3.3}%
\contentsline {subsection}{\numberline {3.4}Mixed correlator holographic functionals $C_{\mathbf {k};\nu |mn}$}{18}{subsection.3.4}%
\contentsline {section}{\numberline {4}Mellin-space functionals}{23}{section.4}%
\contentsline {subsection}{\numberline {4.1}Deriving the $\setbox \z@ \hbox {\mathsurround \z@ $\textstyle B$}\mathaccent "0362{B}_{\mathbf {k};\mathrm {t}|mn}^{s,t}$ functional}{24}{subsection.4.1}%
\contentsline {subsection}{\numberline {4.2}Mellin-space representation of holographic functionals}{27}{subsection.4.2}%
\contentsline {section}{\numberline {5}Applications to the 3D Ising model}{28}{section.5}%
\contentsline {subsection}{\numberline {5.1}Evaluating 3D Ising model sum rules}{29}{subsection.5.1}%
\contentsline {subsubsection}{\numberline {5.1.1}$\langle \sigma \sigma \sigma \sigma \rangle $}{30}{subsubsection.5.1.1}%
\contentsline {subsubsection}{\numberline {5.1.2}$\langle \epsilon \epsilon \epsilon \epsilon \rangle $}{31}{subsubsection.5.1.2}%
\contentsline {subsubsection}{\numberline {5.1.3}$\langle \epsilon \sigma \epsilon \sigma \rangle $}{34}{subsubsection.5.1.3}%
\contentsline {subsubsection}{\numberline {5.1.4}$\langle \epsilon \sigma \sigma \epsilon \rangle $}{36}{subsubsection.5.1.4}%
\contentsline {subsubsection}{\numberline {5.1.5}$\langle \sigma \sigma \epsilon \epsilon \rangle $ and $\langle \epsilon \epsilon \sigma \sigma \rangle $}{37}{subsubsection.5.1.5}%
\contentsline {subsection}{\numberline {5.2}Approximate solutions to crossing from truncated sum rules}{41}{subsection.5.2}%
\contentsline {section}{\numberline {6}Discussion}{43}{section.6}%
\contentsline {section}{\numberline {A}Detailed derivation of the $\mathfrak {B}_{\mathbf {k}|mn}^{\mathfrak {a},\mathfrak {b}}$ kernel}{45}{appendix.A}%
\contentsline {section}{\numberline {B}$\mathfrak {B}_{\mathbf {k}|mn}^{\mathfrak {a},\mathfrak {b}}$ kernel simplification}{46}{appendix.B}%
\contentsline {section}{\numberline {C}Mack Polynomials}{46}{appendix.C}%
\contentsline {section}{\numberline {D}Mixed correlator analytic double-twist functionals}{48}{appendix.D}%
\contentsline {section}{\numberline {E}Varying $v$ for the $\langle \sigma \sigma \sigma \sigma \rangle $ sum rule}{50}{appendix.E}%

